Back to Basics: Unsupervised Learning of Optical Flow via Brightness Constancy and Motion Smoothness

Recently, convolutional networks (convnets) have proven useful for predicting optical flow. Much of this success is predicated on the availability of large datasets that require expensive and involved data acquisition and laborious la- beling. To bypass these challenges, we propose an unsuper- vised approach (i.e., without leveraging groundtruth flow) to train a convnet end-to-end for predicting optical flow be- tween two images. We use a loss function that combines a data term that measures photometric constancy over time with a spatial term that models the expected variation of flow across the image. Together these losses form a proxy measure for losses based on the groundtruth flow. Empiri- cally, we show that a strong convnet baseline trained with the proposed unsupervised approach outperforms the same network trained with supervision on the KITTI dataset.

==> Unsupervised Flow/abstract.tex <==
\begin{abstract}
\vspace{-7pt}Recently, convolutional networks (convnets) have proven useful for predicting optical flow.
%a variety of low-level vision tasks, including optical flow.
Much of this success is predicated on the availability of large datasets that require expensive and involved
data acquisition and laborious labeling.  To bypass these challenges,
%the acquisition and labeling challenges, 
we propose an unsupervised approach (i.e., without 
leveraging groundtruth flow) to train a convnet end-to-end for predicting optical flow between two images.
%Rather than rely on both imagery and the corresponding groundtruth flow for training, we use the images alone.  In particular, 
We use a loss function that combines a data term that measures photometric constancy over time with a spatial
term that models the expected variation of flow across the image. 
Together these losses form a proxy measure for losses based on the groundtruth flow.
Empirically, we show that a strong convnet baseline trained with the proposed unsupervised approach outperforms
the same network trained with supervision on the KITTI dataset. %\todo{All: This last sentence may change depending on results.}
\end{abstract}

==> Unsupervised Flow/contributions.tex <==
\vspace{5pt}\noindent{\bf Contributions } In the light of previous research, we make the following contributions.  First, we present an unsupervised approach to training a convnet in an
end-to-end manner for predicting optical flow between two images.  The limited but valuable  
groundtruth flow is reserved for fine-tuning the network and cross-validating its parameters.
Second, we demonstrate empirically that a strong convnet baseline trained with our unsupervised approach outperforms the same network trained with supervision on KITTI,
where insufficient groundtruth flow is available for training.

==> Unsupervised Flow/evaluation.tex <==
\subsection{Datasets}

%\noindent{\bf Flying Chairs } This synthetic dataset is realized by applying affine mappings to publicly available
%colour images and a rendered set of 3D chair models.  The dataset is comprised of $22, 232$ training 
%and 640 test image pairs with groundtruth flow. %, each with a resolution of $512\times 384$.  
%To cross-validate the hyper-parameters and monitor for
%overfitting in learning, we set aside $2, 000$ image pairs from the training set.  
%We use both photometric and geometric augmentations to avoid overfitting. % in learning. 
%%Unless otherwise stated, the same photometric and geometric augmentations are applied to both images of a pair.
%The photometric augmentations are comprised of additive Gaussian noise applied to each image with a standard deviation sampled uniformly between $0$ and $0.04$,
%contrast sampled between $-0.8$ and $0.4$, multiplicative colour changes to the RGB channels from $0.5$ to $2$, gamma from $0.7$ to $1.5$ and additive
%brightness changes sampled from a Gaussian with a standard deviation of $0.2$.  %The photometric augmentations are   
%%The multiplicative changes are applied to both images
%%of a pair, while the rest of the photometric transformations are applied separately.
%The geometric transformations are comprised of 2D translations
%sampled uniformly between $20\%$ of the horizontal and vertical image dimensions, left-right flipping, 
%rotations between $\pm 17\degree$ and scalings between $0.9$ and $2$.\\ 
%%Additionally, a smaller relative geometric transformation is applied separately to each image.
 
\noindent{\bf Flying Chairs } This synthetic dataset is realized by applying affine mappings to publicly available
colour images and a rendered set of 3D chair models.  The dataset contains $22, 232$ training 
and 640 test image pairs with groundtruth flow.  
To cross-validate the hyper-parameters and monitor for
overfitting in learning, we set aside $2, 000$ image pairs from the training set.  
We use both photometric and geometric augmentations to avoid overfitting. % in learning. 
%Unless otherwise stated, the same photometric and geometric augmentations are applied to both images of a pair.
The photometric augmentations are comprised of additive Gaussian noise applied to each image,
contrast, multiplicative colour changes to the RGB channels, gamma  and additive
brightness.  %The photometric augmentations are   
%The multiplicative changes are applied to both images
%of a pair, while the rest of the photometric transformations are applied separately.
The geometric transformations are comprised of 2D translations, left-right flipping, 
rotations and scalings.\\ 
%Additionally, a smaller relative geometric transformation is applied separately to each image.

% *** This paragraph contains more details about augmentation ***
%\noindent{\bf KITTI 2012 Flow }  This dataset consists of images collected from a driving platform.
%%\todo{All: Depending on time, we may just report results on KITTI 2012.} This benchmark is comprised of two data sets, KITTI 2012 \cite{geiger2013} and KITTI 2015 \cite{Menze2015CVPR}, captured from a moving vehicle.  
%%The ground truth flow is realized by matching temporal point clouds from a 3D range sensor and projecting the 3D flow onto 
%%the image.  Consequently, the ground truth flow is sparse, distant objects are not accounted for and in the case of the 2012 benchmark only rigid elements are captured.
%%KITTI 2015 includes ground truth flow for non-rigid elements (i.e., passing vehicles) by fitting geometrically similar CAD models. 
%There are 194 and 195 training and testing image pairs, respectively, with sparse groundtruth flow.
%The training set is used for cross-validation and to monitor the learning progress.
%For training, we use the raw KITTI data\footnote{KITTI benchmark raw data \url{www.cvlibs.net/datasets/kitti/raw_data.php}} %data that is part of the KITTI 
%%benchmark suite
%from the city, residential and road categories, where groundtruth flow is unavailable.  
%%Some testing images may also be present in the raw data.
%To avoid training on related testing imagery, we remove all raw images that are visually similar with the testing ones, including their 
%temporal neighbours $\pm 20$ frames.  The (curated) raw data is comprised of $82, 958$  image pairs.
%%with no corresponding flow ground truth provided.  
%We include both photometric and geometric augmentations.
%The photometric augmentations are comprised of  
%contrast sampled between $-0.3$ and $0.3$, multiplicative colour changes from $0.9$ to $1.1$.  In addition,
%we include gamma, brightness changes and noise with the same parameters as used with the Flying Chairs dataset.
%The geometric transformations are comprised of scalings between $0.9$ and $1.1$ and left-right flipping applied
%to both images.  Also, we use a relative translation between image pairs 
%sampled uniformly between $5\%$ of the horizontal and vertical image dimensions.
% ******

\noindent{\bf KITTI 2012 }  This dataset consists of images collected on a driving platform.
%\todo{All: Depending on time, we may just report results on KITTI 2012.} This benchmark is comprised of two data sets, KITTI 2012 \cite{geiger2013} and KITTI 2015 \cite{Menze2015CVPR}, captured from a moving vehicle.  
%The ground truth flow is realized by matching temporal point clouds from a 3D range sensor and projecting the 3D flow onto 
%the image.  Consequently, the ground truth flow is sparse, distant objects are not accounted for and in the case of the 2012 benchmark only rigid elements are captured.
%KITTI 2015 includes ground truth flow for non-rigid elements (i.e., passing vehicles) by fitting geometrically similar CAD models. 
There are 194 and 195 training and testing image pairs, respectively, with sparse groundtruth flow.
The training set is used for cross-validation and to monitor the learning progress.
For training, we use the raw KITTI data %\footnote{KITTI benchmark raw data \url{www.cvlibs.net/datasets/kitti/raw_data.php}} %data that is part of the KITTI 
%benchmark suite
from the city, residential and road classes, where groundtruth flow is unavailable.  
%Some testing images may also be present in the raw data.
To avoid training on related testing imagery, we remove all raw images that are visually similar with the testing ones, including their 
temporal neighbours $\pm 20$ frames.  The (curated) raw data is comprised of $82, 958$  image pairs.
%with no corresponding flow ground truth provided.  
We include both photometric and geometric augmentations.
We use the same type of photometric augmentations as applied to Flying Chairs. 
%contrast, multiplicative colour changes, gamma, brightness changes and noise with the same parameters as used with the Flying Chairs dataset.
The geometric transformations consist of left-right flipping and scalings. % between $0.9$ and $1.1$ and left-right flipping applied
%to both images.  
We also use a small relative translation.% between image pairs.
%sampled uniformly between $5\%$ of the horizontal and vertical image dimensions.

% *** This paragraph contains more details about augmentation ***
%\noindent{\bf KITTI Flow} \todo{All: Depending on time, we may just report results on KITTI 2012.} This benchmark is comprised of two data sets, KITTI 2012 \cite{geiger2013} and KITTI 2015 \cite{Menze2015CVPR}, captured from a moving vehicle.  
%The ground truth flow is realized by matching temporal point clouds from a 3D range sensor and projecting the 3D flow onto 
%the image.  Consequently, the ground truth flow is sparse, distant objects are not accounted for and in the case of the 2012 benchmark only rigid elements are captured.
%KITTI 2015 includes ground truth flow for non-rigid elements (i.e., passing vehicles) by fitting geometrically similar CAD models. The 2012 and 2015
%data sets contain 195 (194) and 200 (200) testing (training) image pairs, respectively.  The 194 training image pairs from KITTI 2012 are used as a held-out 
%set for cross validating the hyper-parameters and to monitor the learning progress.
%For training, we use the raw data that is part of the KITTI 
%benchmark suite\footnote{KITTI benchmark raw data \url{www.cvlibs.net/datasets/kitti/raw_data.php}} from the city, residential and road categories.  
%Some testing images may also be present in the raw data.
%To avoid training on related testing imagery, we remove all raw images that are highly visually similar with the testing images and their 
%temporal neighbours with a temporal window of $\pm 20$ frames.  The (curated) raw data is comprised of $82,958$ image pairs
%with no corresponding flow ground truth provided.  In training, we include augmentation in the form of left-right flipping.
%\todo{Kosta, Jason: Add discussion about what we use for the validation set.  For instance, we can say the following.
%For cross-validating and monitoring for overfitting, we use the KITTI training set flow pairs.}
% ******

\subsection{Training details}
We use the ``FlowNet Simple'' architecture provided in the publicly available FlowNet Caffe code \cite{FlowNet}. %\footnote{FlowNet code (v1.0): \url{lmb.informatik.uni-freiburg.de/resources/software.php}}   
%The generalized Charbonnier parameter, $\alpha$, is set to $0.25$ and $0.38$ for the photometric losses on Flying Chairs and KITTI, respectively,
%and $0.37$ and $0.21$ for the smoothness losses.
For the photometric loss, the generalized Charbonnier parameter, $\alpha$, is set to $0.25$ and  $0.38$ for Flying Chairs and KITTI, respectively.
For the smoothness loss, $\alpha$ is set to $0.37$ and $0.21$ for Flying Chairs and KITTI, respectively.
%$\alpha$ is set to $XXX$ for Flying Chairs and $XXX$ for KITTI based on cross-validation.
The smoothness weight, $\lambda$, is set to $1$ for Flying Chairs and $0.53$ for KITTI. % based on cross-validation.
We use Adam as the optimization method, where its parameters $\beta_1=0.9$ and $\beta_2=0.999$.  
%We use Adam as the optimization method, where its parameters $\beta_1$ and $\beta_2$ are set to 
%$0.9$ and $0.999$, respectively.
The initial learning rate is set to 
\num{1.6e-5} 
%$1.6e-5$ 
for Flying Chairs and 
\num{1.0e-5} 
%$1.0e-5$ 
for KITTI and 
we divide it by half every $100,000$ iterations.
The batch size is set to four image pairs.  In total, we train using $600, 000$ iterations for Flying Chairs and $400, 000$ for KITTI.
In initial tests, we noticed that the unsupervised approach had difficulties in regions that were highly saturated or very dark. % in the raw imagery.
Adding photometric augmentation compounds this issue by making these regions even less discriminable.  To address this issue, we pass
the geometrically augmented images directly to the photometric loss prior to photometric augmentation.  Further,
we apply a local $9\times 9$ response normalization to the geometrically augmented images to ameliorate multiplicative lighting factors.

%\todo{Jason: Provide description.}
%\begin{itemize}
%   \item ``FlowNet Simple'' architecture provided in the publicly available FlowNet code\footnote{FlowNet code (v1.0): \url{http://lmb.informatik.uni-freiburg.de/resources/software.php}} 
%   \item Caffe framework
%   \item generalized Charbonnier $\alpha = XXX$
%   \item Adam used as optimization method; $\beta_1 = 0.9$ and $\beta_2 = 0.999$
%   \item the learning rate $\lambda = XXX$
%   \item learning rate schedule, if any 
%   \item the batch size is set to four image pairs  
%   \item number of iterations
%\end{itemize}



\subsection{Results}

Table \ref{table:EPE} provides a summary of results.  As expected,  FlowNet trained with the groundtruth flow on Flying Chairs outperforms the unsupervised one.  Note, however,  the scenario where sufficient dense groundtruth is available is generally unrealistic with real imagery. 
Conversely, KITTI  exemplifies an automative scenario, where abundant dense groundtruth flow with real images is unavailable.  To sidestep this issue, previous work \cite{fischer2015} 
used synthetic data as a proxy for supervised training.
On the non-occluded (NOC) metric, the unsupervised approach improves upon the 
supervised one \cite{fischer2015} on the KITTI training set.  This improvement persists on the official test set.  Considering all pixels (i.e., occluded and non-occluded)
the proposed approach remains competitive to the supervised one.  Figure \ref{fig:flow-example} shows an example flow prediction result on KITTI.
While the performance of the unsupervised approach lags behind the state-of-the-art, it operates in realtime with a testing runtime of 
$0.03$ seconds on an NVIDIA GTX 1080 GPU.%, as compared to the state-of-the-art.

%NVIDIA GTX Titan GPU

%Since the FlowNet architecture is unchanged, the testing runtime remains real-time at $0.08$ seconds on an NVIDIA GTX
%Titan GPU.

%\todo{All: Insert discussion of results here.}

\begin{figure}[t]
\begin{center}
    \epsfig{file=./Img/000044.png, width = 2.9in}
    \epsfig{file=./Img/000044_gt.png, width = 2.9in}
    \epsfig{file=./Img/000044_img1_flow.png, width = 2.9in}
\end{center}
\vspace{-20pt}
\caption{KITTI  example. %Flow prediction example on KITTI. 
(top-to-bottom) Input image frames overlaid, groundtruth flow, and predicted flow from unsupervised network overlaid on the first input image.} 
%\caption{Flow prediction examples. (top) Flying Chairs and (bottom) KITTI.} 
\label{fig:flow-example}
\vspace{-5pt}
\end{figure}

%\begin{figure}[t]
%\begin{center}
%    \epsfig{file=Flying-chairs-examples.pdf, width = 3in}
%\end{center}
%\caption{Flow prediction examples on the KITTI dataset.  \todo{Jason: We will show the two input images overlaid and a comparison with
%FlowNet Simple and our trained model.   Show EPEs for both predictions.}}
%\label{fig:KITTI-example}
%\end{figure}

%
%\begin{table}[t]\begin{center}
%\begin{tabular}{|c|c|c|c|}\hline
%        \multirow{2}{*}{Approach}       &Chairs & \multicolumn{2}{c|}{KITTI 2012}\\\cline{2-4}
%                        &test  &train & test \\\hline\hline
%   EpicFlow \cite{revaud2015}    &2.94& 3.47& 3.8   \\
%   DeepFlow \cite{weinzaepfel2013}  &3.53& 4.58& 5.8   \\
%   LDOF \cite{brox2011}        &3.47& 13.73& 12.4   \\
%   supervised FlowNet \cite{dosovitskiy2015}     &2.71&7.52 &9.1    \\\hline
%   unsupervised FlowNet    & & & \\ \hline   
%\end{tabular}
%\end{center}
%\caption{Average endpoint error (EPE) flow results.  %The EPE of several recent optical flow approaches are shown.
% The reported EPE for supervised FlowNet are the best results of the FlowNet Simple architecture reported previously \cite{dosovitskiy2015}
%without post processing with variational smoothing. \todo{All: We may also include the KITTI 2015 results in this table.}} 
%\end{table}


%\begin{table*}[t]\begin{center}
%\begin{tabular}{|c|c|c|c|c|c|}\hline
%        \multirow{2}{*}{Approach}       &Chairs & \multicolumn{2}{c|}{KITTI 2012}& \multicolumn{2}{c|}{KITTI 2015}\\\cline{2-6}
%                        &test  &train & test&train & test \\\hline\hline
%   EpicFlow \cite{revaud2015}    &2.94& 3.47& 3.8&&   \\
%   DeepFlow \cite{weinzaepfel2013}  &3.53& 4.58& 5.8&&   \\
%   LDOF \cite{brox2011}        &3.47& 13.73& 12.4 &&  \\
%   supervised FlowNet \cite{dosovitskiy2015}     &2.71&7.52 &9.1 &&   \\\hline
%   unsupervised FlowNet    & & &&& \\ \hline   
%\end{tabular}
%\end{center}
%\caption{Average endpoint error (EPE) flow results.  %The EPE of several recent optical flow approaches are shown.
% The reported EPE for supervised FlowNet are the best results of the FlowNet Simple architecture reported previously \cite{dosovitskiy2015}
%without post processing with variational smoothing. \todo{All: Present KITTI2015 if time allows.}} 
%\end{table*}

\begin{table}[t]\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}\hline
        \multirow{3}{*}{Approach}       & \multirow{2}{*}{Chairs} & \multicolumn{4}{c|}{KITTI} \\\cline{3-6}
                        &   &\multicolumn{2}{c|}{Avg.\ All}     &  \multicolumn{2}{c|}{Avg.\ NOC}\\\cline{2-6}
                        &test  &train & test&train & test\\\hline\hline
   EpicFlow \cite{revaud2015}    &2.9& 3.5& 3.8& 1.8& 1.5  \\
   DeepFlow \cite{weinzaepfel2013}  &3.5& 4.6& 5.8& 2.0& 1.5   \\
   LDOF \cite{brox2011}        &3.5& 13.7& 12.4& 5.0& 5.6 \\
   FlowNet \cite{fischer2015}     &2.7&7.5 &9.1& 5.3 &5.0    \\\hline
   FlowNet (ours)    & 5.3 & 11.3 & 9.9 & 4.3 & 4.6 \\ \hline   
\end{tabular}
\end{center}
\vspace{-17pt}
\caption{Average endpoint error (EPE) flow results.  %The EPE of several recent optical flow approaches are shown.
The reported EPEs for supervised FlowNet are the best results of the FlowNet Simple architecture \cite{fischer2015}
without variational smoothing post-processing.
``Avg.\ All'' and ``Avg.\ NOC'' refer to the EPE taken over all the labeled pixels and all non-occluded labeled pixels, respectively.}
% \todo{Jason: Replace results on KITTI training with no occlusion ones.}} 
\label{table:EPE}
\vspace{-10pt}
\end{table}



==> Unsupervised Flow/motivation.tex <==
Visual motion estimation is a core research area of computer vision.  Most prominent has been the recovery of the
apparent motion of image brightness patterns, i.e., optical flow.  Much of this work has centred on extracting the pixelwise
velocities between two temporal images within a variational framework \cite{horn1981,sun2014}.%, where the domain
%knowledge has almost exclusively been integrated into the objective function.

Recently, convolutional networks (convnets) have proven useful for a variety of per-pixel prediction tasks, including optical flow \cite{fischer2015}.
Convnets are high-capacity models that approximate the complex, non-linear transformation between input imagery and the output.  
%Here, domain knowledge is encoded in the weights of the convnet learned from a training set.
%Here, the domain knowledge appears in two forms: the weights of the convnet learned from a dataset, and the particular form of the learning objective.
Success with convnets has relied almost exclusively on fully-supervised schemes, where the target value
(i.e., the label) is provided during training.  This is problematic for learning optical flow because directly obtaining the motion field
groundtruth from real scenes {}\textemdash{} the quantity that optical flow attempts to approximate {}\textemdash{} is not possible.  

In this paper, we propose an end-to-end unsupervised approach to train a convnet for predicting optical flow between two images 
based on a standard variational loss.
Rather than rely on imagery as well as the corresponding groundtruth flow for training, we use the images alone.  In particular,
we use a loss function that combines a data term that measures photometric constancy over time with a spatial
term that models the expected variation of flow across the image. 
%we use the photometric pixelwise disagreement between images and a measure of flow smoothness.
The photometric loss measures the difference between the first input image and the (inverse) warped subsequent image based on the predicted
optical flow by the network.  The smoothness loss measures the difference between spatially neighbouring flow predictions.  Together, these
two losses form a proxy for losses based on the groundtruth flow.


%\noindent{\bf What?}
%\begin{itemize}
%\item in this paper we present an unsupervised approach for training a convolutional network (convnet) for predicting flow from two images 
%\item convnets approximate the complex non-linear transformation between an input imagery and the output
%\item convnets have shown success in a variety of computer vision tasks
%\item they have traditionally been applied to holistic image type tasks but recently have proven useful for per-pixel prediction tasks, such as single view 
%depth estimation \cite{eigen2014}, semantic segmentation \cite{chen2015,long2015} and optical flow estimation \cite{dosovitskiy2015}
%\end{itemize}
%
%\noindent{\bf Why?}
%\begin{itemize}
%\item deep convnets require a vast amount of labeled training data
%\item availability of large labeled data sets has been responsible in part for the recent successes of deep learning in various approaches
%\item generally, obtaining the motion field groundtruth from image sequences is not possible
%\item existing optical flow datasets \cite{baker2011,butler2012,geiger2013} are too small to support training accurate networks
%\item Middlebury \cite{deqing2014} sidesteps this issue by collecting imagery in a controlled lab setting where the objects are painted to support the recovery of groundtruth flow
%\item KITTI \cite{geiger2013} provides sparse flow maps via estimates of the motion field achieved by registering depth maps from a range sensor
%\item Sintel \cite{butler2012} uses computer graphics to generate the imagery and corresponding ground truth flow 
%\end{itemize}
%
%\noindent{\bf How?}
%\begin{itemize}
%\item we present an unsupervised approach to train a convnet for flow prediction from two image frames that sidesteps the requirement of labeled data
%%\item in training, a pair of input images are considered%, we train a convnet to warp one image to the other using the predicted 
%%estimate of optical flow
%\item we use the photometric pixelwise disagreement between the images and a measure of flow smoothness as a proxy for manually labeled flow used in supervised approaches
%\item photometric loss:  difference between the first input image and the (inverse) warped subsequent image based on the predicted optical flow by the network 
%\item smoothness loss: difference between spatially neighbouring flow predictions
%%\item by recasting the flow estimation problem in terms of more classical brightness constancy formulations allows integrating richer loss functions that have been proposed in the past, e.g., natural image priors of flow
%\item this approach is in line with traditional approaches for estimating flow between temporally neighbour image frames
%\item we require no manual annotation
%\item anticipated contributions: we show that our approach to unsupervised learning of flow gives comparable results on the synthetic ``Flying Chairs'' dataset where the generation of training imagery and
%groundtruth flow is limitless and show comparable (or superior results) to that of the state-of-the-art on real imagery, where sufficient groundtruth flow is unavailable
%\end{itemize}

==> Unsupervised Flow/related_work.tex <==
Recovering optical flow between two frames is a well studied problem, with much previous work founded on variational formulations \cite{horn1981,brox2011,sun2014,revaud2015}. %,chen2016}.
%Numerous variants of this formulation have been proposed targeting various aspects of the problem, such as the boundaries
%between moving surfaces and recovering large displacements \cite{brox2011,revaud2015,chen2016}.  
Our loss is similar to the objective functions proposed for two-frame motion estimation; however, rather than 
optimize the velocity map between input frames,
we use it to optimize the convnet weights over the training set of imagery. 
%While traditionally focused on whole image categorization tasks, deep learning methods have recently shown promise on a variety of dense pixel prediction tasks, such as depth (e.g., \cite{}), 
%surface normal (e.g., \cite{}) and semantic segmentation (e.g., \cite{}).

Several recent works \cite{fischer2015,mayer2016} %,teney2016} 
have proposed convnets that learn the 
%complex, non-linear 
mapping between input image frames and the corresponding flow.
Each of these approaches is presented in a supervised setting, where images and their corresponding groundtruth flows are provided.
%In concurrent work \cite{patraucean2015}, a spatiotemporal video auto encoder was introduced that incorporates a long short-term memory (LSTM) architecture for unsupervised
%flow and image frame prediction.  Only preliminary qualitative result were provided.
%Here, we present a simpler feedforward convnet model targeting flow prediction alone.
This setting assumes the availability of a large, annotated dataset. % in each domain of interest. 
%A necessary prerequisite for training these previous convnet architectures for flow prediction
%is a large dataset of temporal imagery with corresponding groundtruth.
%Obtaining flow groundtruth is generally infeasible since it cannot be directly measured.  
Existing flow datasets (e.g., KITTI  \cite{geiger2013}) % \cite{butler2012,geiger2013,deqing2014}
are too small to support training accurate networks.  Computer generated scenes and their corresponding flow \cite{fischer2015,mayer2016,gaidon2016} %,ros2016} 
provide a means to address this issue.
Although some recent efforts have attempted to semi-automate the data creation process \cite{gaidon2016}, creating large, diverse imagery remains laborious.
% however, creating 
%large diverse imagery is laborious, although some recent efforts have attempted to semi-automate the process \cite{gaidon2016}. 
 Another possibility is using the output of an existing optical
flow estimator to provide the groundtruth \cite{tran2016}.  This training approach may result in learning both correct flow prediction and the failure aspects of the flow estimator
used for training.  In this work, we avoid these drawbacks by learning flow in an unsupervised manner, using only  the input imagery. 

Concurrent work has proposed unsupervised methods to circumvent the need of vasts amounts of labeled data for training. %, where such data is difficult to obtain. % via unsupervised methods.
A spatiotemporal video autoencoder \cite{patraucean2015} was introduced that incorporates a long short-term memory (LSTM) architecture for unsupervised
flow and image frame prediction.  %Only preliminary qualitative results were provided.
Here, we present a simpler feedforward convnet model targeting flow prediction alone.
Most closely related to the current paper is recent work that proposed a convnet for depth estimation trained in an unsupervised manner \cite{garg2016}.  In a similar fashion to the proposed approach, a  photometric loss warps one image to another, and a smoothness loss term is used to bias the predictor towards smooth depth estimates.
Unlike the current work, the manner in which the photometric loss is handled (via a linear Taylor series approximation) precludes end-to-end learning.

%\noindent{\bf Optical flow}
%\begin{itemize}
%\item variational approaches have dominated optical flow estimation benchmarks \cite{horn1981}
%\item discuss traditional approach to optical flow estimation \cite{horn1981,lucas1981,deqing2014}
%\item more recent work have concentrated efforts on recovering large displacements \cite{brox2011,revaud2015}
%\end{itemize}

%\noindent{\bf Training}
%\begin{itemize}
%\item laborious, difficult to capture the full diversity of the real-world from computer graphics
%\item train from the output of a handcrafted optical flow method; using an existing flow estimator does pose the risk
%of learning the biases of the estimator (e.g., failure modes)
%\item discuss approach to generating training data synthetically; difficult to capture the full variability of real world images and to data generating 
%diverse instances requires human intervention, cite Brox papers \cite{dosovitskiy2015,mayer2016} and CVPR2016 papers
%\item discuss using the output of an existing handcrafted flow estimator as the supervisory signal \cite{tran2016}
%\item synthetic datasets \cite{gaidon2016,ros2016}
%\end{itemize}
%
%\noindent{\bf CNN}
%\begin{itemize}
%\item supervised CNNs for flow \cite{dosovitskiy2015,teney2016,tran2016}
%\item unsupervised single view depth estimation\cite{garg2016}
%\end{itemize}
%
%\noindent{\bf Unsupervised}
%\begin{itemize}
%\item previous efforts with supervised learning of motion between videos using neural networks \cite{taylor2010,konda2013}
%\item end-to-end here we use the cost function used by traditional approaches but solve for flow in a feedforward manner (see ``Single Image 3D Interpreter Network'')
%\item \cite{garg2016}
%\end{itemize}
%
%\begin{itemize}
%\item we use a spatial transformer network \cite{jaderberg2015} to warp our images based on the predicted optical flow 
%%\item can integrate statistics of optical flow into loss function \cite{roth2005}
%\end{itemize}

==> Unsupervised Flow/summary.tex <==
We presented an end-to-end unsupervised approach to training convnets for optical flow prediction. 
%\todo{All: This next sentence may change depending on results.} 
%Using the proposed unsupervised training approach, 
We showed that the proposed unsupervised training approach yields competitive and even superior performance
to a supervised one. % on the same network.  
This opens up avenues for further improvement by 
leveraging the vast amounts of video that can easily be captured with commodity cameras taken in the domain of interest, such as automotive applications.
Furthermore, this is a general learning framework that can be extended in a variety of ways via more sophisticated losses
%For instance, one can more discriminative photometric term(s) and a more expressive spatial loss based on the natural or application-specific spatial statistics of flow \cite{sun2008}.
to enhance convnet-based mappings between temporal input imagery and flow.


%\begin{itemize}
 %  \item This is a general learning framework that can be extended with richer priors (e.g., natural spatial statistics of flow \cite{roth2005,sun2008}) to enhance the CNN-based mapping approximator
%   between temporal input imagery and flow.
  % \item here we have considered a homogeneous (smoothness) prior, but one could integrate inhomogeneous models to reflect different spatial characteristics of flow in the target application (e.g., automotive)
%\end{itemize}

==> Unsupervised Flow/technical_approach.tex <==
Given an RGB image pair as input, $\mathbf{X} \in \mathbb{R}^{H\times W \times 6}$, our objective is to learn a non-linear mapping (approximated by a convnet) 
to the corresponding optical flow, $\mathbf{Y} \in \mathbb{R}^{H\times W \times 2}$, where $H$ and $W$ denote the image height and width, respectively.
In Section \ref{sec:loss}, we outline our unsupervised loss.  Section \ref{sec:architecture} provides details on how the unsupervised loss is integrated with a 
reference convnet architecture.

\subsection{Unsupervised loss} \label{sec:loss}
%\begin{align}
 % E(\mathbf{u}, \mathbf{v}) =& \sum_{i,j}\{ \rho_D(I(i,j,t) - I(i + u_{i,j}, j + v_{i,j}, t+1)) \nonumber\\ 
%   & + \lambda[\rho_{S} (u_{i,j} - u_{i+1,j})  + \rho_{S} (u_{i,j} - u_{i,j+1}) \nonumber\\  
  % & + \rho_{S} (v_{i,j} - v_{i+1,j}) + \rho_{S} (v_{i,j} - v_{i,j+1}) \},
%\end{align}
%where $I$ denotes the input image sequence, $\mathbf{u}$ and $\mathbf{v}$ are the horizontal and vertical components of the optical flow field to be estimated, $\lambda$ is a regularization parameter, and 
%$\rho_D$ and $\rho_S$ are the data and spatial penalty functions.  In this work, we consider the robust generalized Charbonnier penalty function $\rho = (x^2 + \epsilon^2)^\alpha$.

The training set is comprised of pairs of temporally consecutive images, $\{ I(x,y,t), I(x,y,t+1)\}$.  Unlike prior work, we do not assume access to the corresponding velocity pixel labels, cf.\ \cite{fischer2015}.
Instead, we return to traditional means for scoring a given solution, via a loss that combines a photometric loss 
between the first image and the warped second image, and a loss related to the smoothness of the velocity field prediction \cite{horn1981}:
\begin{align}
 \mathcal{L}&(\mathbf{u}, \mathbf{v}; I(x,y,t), I(x,y,t+1)) = \nonumber\\
  &\ell_\text{photometric} (\mathbf{u}, \mathbf{v}; I(x,y,t), I(x,y,t+1)) + \nonumber\\
  &\lambda \ell_\text{smoothness} (\mathbf{u}, \mathbf{v}), \label{eq:loss}
\end{align}
where %$I$ denotes the input image sequence, 
$\mathbf{u}, \mathbf{v} \in \mathbb{R}^{H\times W}$ are the horizontal and vertical components of the predicted flow field, respectively, and $\lambda$ is a regularization parameter
that weighs the relative importance of smoothness of the predicted flow.  Note, the photometric loss can be replaced or augmented with other measures, 
such as the image gradient constancy \cite{brox2011}. 
%see \cite{derpanis2006}
%for a survey of photometric constancy assumptions. 

Given the predicted flow, the photometric loss is computed as the difference between the first image and the backward/inverse warped second image:% with bilinear interpolation
%as the difference between the images
%Given the predicted flow, we backward warp the second image with bilinear interpolation to the first and compute the photometric loss as the difference between the images:
\begin{align}
    \ell&_\text{photometric} (\mathbf{u}, \mathbf{v}; I(x,y,t), I(x,y,t+1)) = \\\nonumber &\sum_{i,j} \rho_D(I(i,j,t) - I(i + u_{i,j}, j + v_{i,j}, t+1)),
\end{align}
where $\rho_D$ is the data penalty function.
We consider the robust generalized Charbonnier penalty function $\rho(x) = (x^2 + \epsilon^2)^\alpha$ to mitigate the effects of outliers \cite{sun2014}.

To compute the non-rigid backward warp, we use the recently proposed spatial transformer module \cite{jaderberg2015}. 
This allows the learning to be performed with standard backpropagation
in an end-to-end fashion.
In brief, the spatial transformer can be described as two parts that work in sequence: (i) a sampling grid generator and (ii) a differentiable image sampler. (The spatial 
transformer localization step is not needed here as flow prediction, $(u,v)$, provides the necessary parameters for the mapping between image points across frames.)  The sampling grid is generated by
the following pointwise transformation:
\begin{equation}
   \begin{pmatrix}
      x_2 \\ y_2   
      \end{pmatrix} = 
      W_{(u, v)}  \begin{pmatrix} x_1 \\ y_1   \end{pmatrix} =  \begin{pmatrix} x_1 + u \\ y_1 + v   \end{pmatrix},
\end{equation}
where $(x_1, y_1)$ are the coordinates in the first image and $(x_2, y_2)$ are the sampling coordinates in the second image. 
The bilinear sampling step can be written in the following \mbox{(sub-)differentiable} form:
\begin{align}
%   I&_\text{warp}(x_i^1,y_i^1,t+1) = \\\nonumber &\sum_n^H\sum_m^WI(m, n, t+1)\max(0,1 - |x_i^2-m|)\max(0,1 - |y_i^2-n|),
   I&_\text{warp}(x_1,y_1,t+1) = \nonumber\\ &\sum_j^H\sum_i^WI(i, j, t+1)M(1 - |x_2-i|)M(1 - |y_2-j|),
\end{align}
where $M(\cdot) = \max(0, \cdot)$. %, and $H$ and $W$ denote the height and width of the grid, respectively.
For details about backpropagating through this module, see \cite{jaderberg2015}.

%The photometric loss alone is insufficient to render a unique flow solution.  
Regions with insufficient image structure support 
multiple equally scoring velocities, e.g., the aperture problem.  To address this ambiguity, we introduce a standard robust (piecewise) smoothness loss: 
\begin{align}
 \ell&_\text{smoothness} (\mathbf{u}, \mathbf{v}) =\nonumber\\
   &  \sum_j^H\sum_i^W [\rho_{S} (u_{i,j} - u_{i+1,j})  + \rho_{S} (u_{i,j} - u_{i,j+1}) \nonumber\\  
   & + \rho_{S} (v_{i,j} - v_{i+1,j}) + \rho_{S} (v_{i,j} - v_{i,j+1})],
   \end{align}
where $\rho_S(\cdot)$ is the (spatial) smoothness penalty function realized by
the generalized Charbonnier function. %As with the photometric loss term, 
%We use the robust generalized Charbonnier function
%for the spatial penalty function.% $\rho = (x^2 + \epsilon^2)^\alpha$. 

A summary of our proposed unsupervised approach for flow prediction is provided in Fig.\ \ref{fig:overview}.

\begin{figure}[t]
\begin{center}
    \epsfig{file=loss-architecture2, width = 3.2in}
\end{center}
\vspace{-20pt}
\caption{Overview of our unsupervised  approach.}% to unsupervised learning of optical flow.}
\label{fig:overview}
\vspace{-10pt}
\end{figure}

  
\subsection{Network architecture}  \label{sec:architecture}
%To demonstrate our proposed approach to unsupervised learning, 
We use ``FlowNet Simple'' \cite{fischer2015} as a reference network.
This architecture consists of a 
%can be described as a two stage process, a 
contractive part followed by an expanding part.  
%The contractive part takes as input two RGB images stacked together. 
%Processing proceeds with a sequence of convolutional layers with a stride of two in several of the layers and ReLU nonlinearities after each layer.
The contractive part takes as
input two RGB images stacked together, and processes them with a cascade of strided convolution layers.
The expanding part implements a ``skip-layer'' architecture that combines information from various levels of the contractive part with ``upconvolving'' layers to iteratively refine the coarse flow predictions.  The FlowNet Simple architecture is illustrated in Fig.\ \ref{fig:flownet_architecture}.

In this work, we use a loss comprised of a final  loss and several intermediate losses placed at various stages of the expansionary part.  The intermediate losses 
are meant to guide earlier layers more directly towards the final objective \cite{lee2015}.  
%This form of loss has been shown to improve convergence and test performance in a variety 
%of tasks (e.g., \cite{lee2015,xie2015}). % and
%is provided in the publicly available FlowNet code.  
In FlowNet, the endpoint error (EPE), a standard error measure for optical flow, is used as the supervised training loss.  As a proxy
to per-pixel groundtruth flow, we replace the EPE with the proposed unsupervised loss, (\ref{eq:loss}).


\begin{figure}[t]
\begin{center}
    \epsfig{file=flow_blocks12, width =2.9in}
    \end{center}
 \vspace{-20pt}
\caption{``FlowNet Simple'' architecture. Two images are taken as input, and an optical flow prediction is generated using a multi-stage refinement process.
Feature maps from the contractive part, as well as intermediate flow predictions, are used in the ``upconvolutional'' part.}
\label{fig:flownet_architecture}
\vspace{-10pt}
\end{figure}
   
   

==> Unsupervised Flow/todo.tex <==
\noindent The following list is meant to summarize possible directions for {\bf future work}.
\begin{enumerate}
\item incorporate the gradient constancy constraint \cite{nagel1983b,haralick1983,tretiak1984,brox2004}:
\begin{align}
    \ell&_\text{gradient} (\mathbf{u}, \mathbf{v}; I(x,y,t), I(x,y,t+1)) = \\\nonumber &\sum_{i,j} \rho_D(\nabla I(i,j,t) - \nabla I(i + u_{i,j}, j + v_{i,j}, t+1)),
\end{align}
where $\rho_D$ is the data penalty function.
   \item incorporate boundary evidence into smoothness loss, so called {\it adaptive image-based regularization}
   \begin{itemize}
      \item so far we have considered a homogeneous, isotropic smoothness term:
      \begin{align}
 \ell&_\text{smoothness} (\mathbf{u}, \mathbf{v}) =\nonumber\\
   &  \lambda\sum_j^H\sum_i^W [\rho_{S} (u_{i,j} - u_{i+1,j})  + \rho_{S} (u_{i,j} - u_{i,j+1}) \nonumber\\  
   & + \rho_{S} (v_{i,j} - v_{i+1,j}) + \rho_{S} (v_{i,j} - v_{i,j+1}) \},
   \end{align}
   where $\rho_S$ is the smoothness penalty function.
 \item       One can also incorporate image evidence
      and realize an inhomogeneous isotropic or anisotropic smoothness term
      \item in real-world imagery, photometric discontinuities typical co-occur with object and motion field boundaries
      \item inhomogeneous isotropic smoothness \cite{weickert2001,wedel2009,xu2012}:       
         
\begin{align}
 \ell&_\text{smoothness} (\mathbf{u}, \mathbf{v}; I(x, y, t)) =   w(i,j; I(x, y, t))\nonumber\\
   &\lambda\sum_j^H\sum_i^W  [\rho_{S} (u_{i,j} - u_{i+1,j})  + \rho_{S} (u_{i,j} - u_{i,j+1}) \nonumber\\  
   & + \rho_{S} (v_{i,j} - v_{i+1,j}) + \rho_{S} (v_{i,j} - v_{i,j+1}) \},
\end{align}
where 
\begin{equation}
 w(i,j; I(x, y, t)) = \exp(-\alpha \| \nabla I(i,j,t) \|^\beta).  \nonumber
\end{equation}
This prior tends to preserve motion discontinuities in regions where the image gradient is high.
 \item inhomogeneous anisotropic smoothness \cite{nagel1983,weickert2001}: 
   \begin{equation}
      \Psi(\nabla u^\top D(\nabla I)\nabla u) +  \Psi(\nabla v^\top D(\nabla I)\nabla v), 
   \end{equation}
   where 
   \begin{equation}
      D(\nabla) = \frac{1}{\|\nabla I \|^2 + 2\lambda^2}(\nabla I^\bot\nabla I^{\bot\top} + \lambda^2\mathbf{I}_{2\times 2}),
   \end{equation}
   where $ I^{\bot}$ denotes the vector perpendicular to the image gradient, $\nabla I$, and $\mathbf{I}_{2\times 2}$ is a $2 \times 2$
   identity matrix. This smoothing term prefers smoothing perpendicular to the gradient while preserving discontinuities 
   across the across the gradient
     \item one can also replace the gradient as a signal for boundaries with a modern boundary detector, e.g., \cite{kokkinos2015}; this should improve performance
   \end{itemize}
  \item visualize (PCA) semantic embedding on raw KITTI to see if incorporating Adam's embedding is plausible
  \item visualize output of modern boundary detector on raw KITTI, e.g., \cite{kokkinos2015}, to see if incorporating the boundary detector outputs
  into an adaptive image-based regularizer is plausible; note that EpicFlow \cite{revaud2015} incorporates a modern boundary detector, i.e., SED
   \item incorporate semantic loss by way of warping Adam's embeddings
   \item incorporate segmentation-aware convolution
   \item evaluate on KITTI 2015
\end{enumerate}



==> todo.tex <==
\noindent The following list is meant to summarize possible directions for {\bf future work}.
\begin{enumerate}
\item incorporate the gradient constancy constraint \cite{nagel1983b,haralick1983,tretiak1984,brox2004}:
\begin{align}
    \ell&_\text{gradient} (\mathbf{u}, \mathbf{v}; I(x,y,t), I(x,y,t+1)) = \\\nonumber &\sum_{i,j} \rho_D(\nabla I(i,j,t) - \nabla I(i + u_{i,j}, j + v_{i,j}, t+1)),
\end{align}
where $\rho_D$ is the data penalty function.
   \item incorporate boundary evidence into smoothness loss, so called {\it adaptive image-based regularization}
   \begin{itemize}
      \item so far we have considered a homogeneous, isotropic smoothness term:
      \begin{align}
 \ell&_\text{smoothness} (\mathbf{u}, \mathbf{v}) =\nonumber\\
   &  \lambda\sum_j^H\sum_i^W [\rho_{S} (u_{i,j} - u_{i+1,j})  + \rho_{S} (u_{i,j} - u_{i,j+1}) \nonumber\\  
   & + \rho_{S} (v_{i,j} - v_{i+1,j}) + \rho_{S} (v_{i,j} - v_{i,j+1}) \},
   \end{align}
   where $\rho_S$ is the smoothness penalty function.
 \item       One can also incorporate image evidence
      and realize an inhomogeneous isotropic or anisotropic smoothness term
      \item in real-world imagery, photometric discontinuities typical co-occur with object and motion field boundaries
      \item inhomogeneous isotropic smoothness \cite{weickert2001,wedel2009,xu2012}:       
         
\begin{align}
 \ell&_\text{smoothness} (\mathbf{u}, \mathbf{v}; I(x, y, t)) =   w(i,j; I(x, y, t))\nonumber\\
   &\lambda\sum_j^H\sum_i^W  [\rho_{S} (u_{i,j} - u_{i+1,j})  + \rho_{S} (u_{i,j} - u_{i,j+1}) \nonumber\\  
   & + \rho_{S} (v_{i,j} - v_{i+1,j}) + \rho_{S} (v_{i,j} - v_{i,j+1}) \},
\end{align}
where 
\begin{equation}
 w(i,j; I(x, y, t)) = \exp(-\alpha \| \nabla I(i,j,t) \|^\beta).  \nonumber
\end{equation}
This prior tends to preserve motion discontinuities in regions where the image gradient is high.
 \item inhomogeneous anisotropic smoothness \cite{nagel1983,weickert2001}: 
   \begin{equation}
      \Psi(\nabla u^\top D(\nabla I)\nabla u) +  \Psi(\nabla v^\top D(\nabla I)\nabla v), 
   \end{equation}
   where 
   \begin{equation}
      D(\nabla) = \frac{1}{\|\nabla I \|^2 + 2\lambda^2}(\nabla I^\bot\nabla I^{\bot\top} + \lambda^2\mathbf{I}_{2\times 2}),
   \end{equation}
   where $ I^{\bot}$ denotes the vector perpendicular to the image gradient, $\nabla I$, and $\mathbf{I}_{2\times 2}$ is a $2 \times 2$
   identity matrix. This smoothing term prefers smoothing perpendicular to the gradient while preserving discontinuities 
   across the across the gradient
     \item one can also replace the gradient as a signal for boundaries with a modern boundary detector, e.g., \cite{kokkinos2015}; this should improve performance
   \end{itemize}
  \item visualize (PCA) semantic embedding on raw KITTI to see if incorporating Adam's embedding is plausible
  \item visualize output of modern boundary detector on raw KITTI, e.g., \cite{kokkinos2015}, to see if incorporating the boundary detector outputs
  into an adaptive image-based regularizer is plausible; note that EpicFlow \cite{revaud2015} incorporates a modern boundary detector, i.e., SED
   \item incorporate semantic loss by way of warping Adam's embeddings
   \item incorporate segmentation-aware convolution
   \item evaluate on KITTI 2015
\end{enumerate}


